Revisiting Fundamentals of Experience Replay

Experience replay is central to off-policy algorithms in deep reinforcement learning (RL), but there remain significant gaps in our understanding. We therefore present a systematic and extensive analysis of experience replay in Q-learning methods, focusing on two fundamental properties: the replay capacity and the ratio of learning updates to experience collected (replay ratio). Our additive and ablative studies upend conventional wisdom around experience replay -- greater capacity is found to substantially increase the performance of certain algorithms, while leaving others unaffected. Counterintuitively we show that theoretically ungrounded, uncorrected n-step returns are uniquely beneficial while other techniques confer limited benefit for sifting through larger memory. Separately, by directly controlling the replay ratio we contextualize previous observations in the literature and empirically measure its importance across a variety of deep RL algorithms. Finally, we conclude by testing a set of hypotheses on the nature of these performance benefits.

==> contribution_1_buffer_nstep.tex <==
% Prajit, I incorporated much of your section into the main paper
\section{Experience replay capacity and n-step returns}
Earlier work which found that larger replay buffers are detrimental to performance \citep{zhang2017deeperlook}.
Both smaller and larger replay buffers were found to negatively impact performance on a set three tasks: a gridworld, Lunar Lander \citep{catto2011box2d} and Pong from the Atari Learning Environment \citep{bellemare2013arcade}.


\subsection{Increasing replay buffer}

% (do we do Rainbow or DQN?)
% Rainbow:
%  - this is the SOTA algorithm, so benefits are non-trivial

% DQN:
%  - simple one, not super complicated so seems reasonable to increase buffer size

We increase the replay capacity by a factor of 10x, from 1M to 10M frames. No other hyperparameters are tuned. In DQN, after the buffer is full, changing the buffer size does not affect the number of times an example is trained on because for a replay buffer of size $N$ and a batch size of $B$, $N * B / N = B$.

Increasing the replay buffer on Rainbow seems to help (+41\%). 
However, when applied to DQN, there are no gains over the baseline (-1\%).
DQN is just a basic version of Rainbow, which suggests one or many of the components added to Rainbow is a factor in better performance due to larger replay capacity.
In particular, the differences between DQN and Rainbow (as implemented in the Dopamine framework) are:
\begin{itemize}
    \item Prioritized Experience Replay (PER): a scheme for sampling non-uniformly from the replay buffer based on upweighting examples that have high TD error. This contrasts to DQN uniform sampling
    \item Adam:  a more powerful optimizer instead of RMSProp, can be loosely viewed as RMSProp with a momentum term
    \item C51: distributional RL, instead of viewing future return as a single scalar to be estimated, estimate the distribution of possible future returns 
    \item n-step returns: instead of regressing towards the one step TD-error: $r_t + \max\limits{a}Q(s_{t+1}, a)$, regress towards an unrolled TD-error $\sum\limits{i=0}{n - 1}r_{t + i} + \max\limits{a}Q(s_{t+n}, a)$. Can be viewed as a tradeoff between the bias of one-step TD estimates and variance of full Monte Carlo rollouts.
\end{itemize}

Rainbow \citep{hessel2018rainbow} demonstrated that these techniques additively improve the policy.
To better understand the effects of each component, we perform both a series of ablations on Rainbow and a series of additions on DQN.
The results are summarized in Table \ref{tab: additive_ablative_analysis}.

\begin{table}[]
    \begin{tabular}{lcccc}
                        & PER   & Adam  & C51   & n-step \\ \hline
    Add to DQN          & 0\%  & +2\%  & -3\%  & \textbf{+23\%}  \\
    Ablate from Rainbow & +28\% & +40\% & +24\% & \textbf{-4\%}  
    \end{tabular}
    \label{tab: additive_ablative_analysis}
    \caption{Additive and ablative studies to measure the impact of four Rainbow improvements to benefit from large replay buffers. The median performance improvement is recorded for each algorithm}
\end{table}

The results indicate that n-step returns is the important component for taking advantage of a larger buffer.
When n-step is removed from Rainbow, a 10x larger experience replay capacity size offers no benefit over the smaller capacity.
Removing any other components still enables the partial Rainbow agent to improve with larger capacity.
Furthermore, n-step is the only component that enables DQN to improve with a larger capacity. 

Another surprising finding is that prioritized experience replay (PER) does not significantly affect the ability to take advantage of a larger capacity.
Intuitively, one would expect PER to become more important in the larger capacity as the probability of sampling an important transition with a uniform sampling policy is reduced with larger capacity. 

\begin{table}[]
    \begin{tabular}{lccc}
                               & $n = 3$   & $n = 5$  & $n = 7$ \\ \hline
    DQN relative improvement          & 23\%  & 30\%  & 44\%  \\
    \end{tabular}
    \label{tab: DQN_n_step}
    \caption{Median performance improvement for the DQN-n-step algorithm varying the $n$-step length.}
\end{table}

We further experiment with increasing $n$ in Table \ref{tab: DQN_n_step} for DQN. 
Increasing $n$ results in larger relative improvements with increased capacity.
This result further strengthens the likelihood of a critical relationship between the $n$-step returns and ability to take advantage of larger experience replay capacity.

